Galactic Chemical Evolution Models Favor an Extended Type Ia Supernova Delay-Time Distribution

Type Ia supernovae (SNe Ia) produce most of the Fe-peak elements in the Universe and therefore are a crucial ingredient in galactic chemical evolution models. SNe Ia do not explode immediately after star formation, and the delay-time distribution (DTD) has not been definitively determined by supernova surveys or theoretical models. Because the DTD also affects the relationship among age, [Fe/H], and [$\alpha$/Fe] in chemical evolution models, comparison with observations of stars in the Milky Way is an important consistency check for any proposed DTD. We implement several popular forms of the DTD in combination with multiple star formation histories for the Milky Way in multi-zone chemical evolution models which include radial stellar migration. We compare our predicted interstellar medium abundance tracks, stellar abundance distributions, and stellar age distributions to the final data release of the Apache Point Observatory Galactic Evolution Experiment (APOGEE). We find that the DTD has the largest effect on the [$\alpha$/Fe] distribution: a DTD with more prompt SNe Ia produces a stellar abundance distribution that is skewed toward a lower [$\alpha$/Fe] ratio. While the DTD alone cannot explain the observed bimodality in the [$\alpha$/Fe] distribution, in combination with an appropriate star formation history it affects the goodness of fit between the predicted and observed high-$\alpha$ sequence. Our model results favor an extended DTD with fewer prompt SNe Ia than the fiducial $t^{-1}$ power law.

==> showyourwork-metadata.tex <==

                \OnGithubActionstrue
                \def\syw@url{https://github.com/lodubay/galactic-dtd}
        \def\syw@slug{lodubay/galactic-dtd}
        \def\syw@sha{b9d5f5053d0b0e2724f3e2b5ab4686eea1fe805c}
        \def\syw@runid{9894213423}

                \AddStampfalse
                \newcommand{\syw@stampX}{1.0}
        \newcommand{\syw@stampY}{1.0}
        \newcommand{\syw@stampSize}{0.75}
        \newcommand{\syw@stampAngle}{-20}
        \newcommand{\syw@stampText}{}
        \newcommand{\syw@stampVersion}{dev}

                        \definecolor{github-icon}{rgb}{0.12,0.47,0.71}
                \definecolor{sandbox-icon}{rgb}{0.80,0.14,0.19}
                \definecolor{cache-icon}{rgb}{0.12,0.47,0.71}
                \definecolor{dataset-icon}{rgb}{0.12,0.47,0.71}
                
                \addvalue{fig:dtds_script}{src/scripts/delay_time_distributions.py}
                \addvalue{fig:sfhs_script}{src/scripts/star_formation_histories.py}
                \addvalue{fig:sfhs_datasetOne}{https://zenodo.org/records/12207380}
                \addvalue{fig:onezone-threepanel_script}{src/scripts/onezone_threepanel.py}
                \addvalue{fig:onezone-twopanel_script}{src/scripts/onezone_twopanel.py}
                \addvalue{fig:feh-df-comparison_script}{src/scripts/feh_df_comparison.py}
                \addvalue{fig:feh-df-comparison_datasetOne}{https://zenodo.org/records/12207380}
                \addvalue{fig:ofe-df-sfh_script}{src/scripts/ofe_df_sfh.py}
                \addvalue{fig:ofe-df-sfh_datasetOne}{https://zenodo.org/records/12207380}
                \addvalue{fig:ofe-df-dtd_script}{src/scripts/ofe_df_dtd.py}
                \addvalue{fig:ofe-df-dtd_datasetOne}{https://zenodo.org/records/12207380}
                \addvalue{fig:ofe-bimodality_script}{src/scripts/ofe_bimodality_summary.py}
                \addvalue{fig:ofe-bimodality_datasetOne}{https://zenodo.org/records/12207380}
                \addvalue{fig:ofe-feh-sfh_script}{src/scripts/ofe_feh_sfh.py}
                \addvalue{fig:ofe-feh-sfh_datasetOne}{https://zenodo.org/records/12207380}
                \addvalue{fig:ofe-feh-dtd_script}{src/scripts/ofe_feh_dtd.py}
                \addvalue{fig:ofe-feh-dtd_datasetOne}{https://zenodo.org/records/12207380}
                \addvalue{fig:ofe-feh-twoinfall_script}{src/scripts/ofe_feh_twoinfall.py}
                \addvalue{fig:ofe-feh-twoinfall_datasetOne}{https://zenodo.org/records/12207380}
                \addvalue{fig:age-ofe-sfh_script}{src/scripts/age_ofe_sfh.py}
                \addvalue{fig:age-ofe-sfh_datasetOne}{https://zenodo.org/records/12207380}
                \addvalue{fig:age-ofe-dtd_script}{src/scripts/age_ofe_dtd.py}
                \addvalue{fig:age-ofe-dtd_datasetOne}{https://zenodo.org/records/12207380}
                \addvalue{fig:analytic-dtds_script}{src/scripts/analytical_dtd_twopanel.py}
                \addvalue{fig:radial-migration_script}{src/scripts/radial_migration.py}
                \addvalue{fig:radial-migration_datasetOne}{https://zenodo.org/records/12207380}
                \addvalue{fig:midplane-distance_script}{src/scripts/midplane_distance.py}
                \addvalue{fig:midplane-distance_datasetOne}{https://zenodo.org/records/12207380}
        
                % \addvalue{output/apogee_regions_table.tex_rule}{Snakefile\#L146}
                \addvalue{output/apogee_regions_table.tex_script}{src/scripts/apogee_regions_table.py}
                \addvalue{output/apogee_regions_table.tex_datasetOne}{https://zenodo.org/records/12207380}
                % \addvalue{output/summary_table.tex_rule}{Snakefile\#L130}
                \addvalue{output/summary_table.tex_script}{src/scripts/summary_table.py}
                \addvalue{output/summary_table.tex_datasetOne}{https://zenodo.org/records/12207380}
                % \addvalue{output/scores_table.tex_rule}{Snakefile\#L138}
                \addvalue{output/scores_table.tex_script}{src/scripts/scores_table.py}
                \addvalue{output/scores_table.tex_datasetOne}{https://zenodo.org/records/12207380}
                \addvalue{output/age_sample_size.txt_script}{src/scripts/age_sample_size.py}
                \addvalue{output/age_sample_size.txt_datasetOne}{https://zenodo.org/records/12207380}
                \addvalue{output/sample_size.txt_script}{src/scripts/age_sample_size.py}
                \addvalue{output/sample_size.txt_datasetOne}{https://zenodo.org/records/12207380}
        
        \renewcommand\showkeyslabelformat[1]{%
        \normalfont%
        \setstackgap{S}{0pt}
        \Shortstack[c]{
            \IfEq*{\usevalue{#1_cache}}{KEYNOTFOUND}{}{\syw@Cache{#1_cache}}
            \IfEq*{\usevalue{#1_datasetThree}}{KEYNOTFOUND}{}{\syw@DatasetThree{#1_datasetThree}}
            \IfEq*{\usevalue{#1_datasetTwo}}{KEYNOTFOUND}{}{\syw@DatasetTwo{#1_datasetTwo}}
            \IfEq*{\usevalue{#1_datasetOne}}{KEYNOTFOUND}{}{\syw@DatasetOne{#1_datasetOne}}
            \IfEq*{\usevalue{#1_script}}{KEYNOTFOUND}{}{\syw@Script{#1_script}}
        }
        % Link to the line in the Snakefile that generates a given variable
        % in the texfile
        \IfEq*{\usevalue{#1_rule}}{KEYNOTFOUND}{}{\syw@Variable{#1_rule}}
        }
        


==> showyourwork.tex <==
% Imports
\RequirePackage{mathtools} % equation tags
\RequirePackage{xcolor} % custom colors
\RequirePackage{hyperref} % url links
\RequirePackage{suffix} % allows definition of starred commmands
\RequirePackage{fontawesome5} % FontAwesome symbols
\RequirePackage{letltxmacro} % command redefinitions
\RequirePackage{xstring} % string manipulation
\RequirePackage{catchfile} % read file into macro
\RequirePackage{totcount} % count total number of errors
\RequirePackage[notref, notcite]{showkeys} % get label refs
\RequirePackage{xspace} % better spacing after icons
\RequirePackage{graphicx} % includegraphics
\RequirePackage{stackengine} % stacking figure links
\RequirePackage{tikz} % stamp
\RequirePackage{etoolbox} % ifcsmacro
\RequirePackage{eso-pic} % AddToShipoutPictureBG
\usetikzlibrary{calc}
\usetikzlibrary{math}
\usetikzlibrary{decorations.text}

% Is this running on GitHub Actions?
\newif\ifOnGithubActions

% Should we add a showyourwork stamp?
\newif\ifAddStamp

% Key-value pairs used to assemble the hyperlinks for figures
% See https://tex.stackexchange.com/a/48931
\def\addvalue#1#2{\expandafter\gdef\csname syw@data@\detokenize{#1}\endcsname{#2}}
\def\usevalue#1{%
  \ifcsname syw@data@#1\endcsname%
    \csname syw@data@#1\expandafter\endcsname%
  \else%
    KEYNOTFOUND%
  \fi%
}

% Import metadata
\IfFileExists{./showyourwork-metadata.tex}{
  \input{showyourwork-metadata.tex}
}{
  \OnGithubActionsfalse
  \AddStampfalse
  \def\syw@url{https://github.com/showyourwork/showyourwork-example}
  \def\syw@sha{dev}
  \def\syw@runid{0}
}

% Log figure script commands (a no-op in the build step)
\newcommand\script[1]{}

% Showyourwork logo
\newcommand{\showyourwork}{%
  \smash{\raisebox{-1.4ex}{\includegraphics[width=7.3em]{showyourwork-logo.pdf}}}\xspace%
}

% Define custom stamp colors
\definecolor{sywStampRed}{rgb}{0.80,0.45,0.45}
\definecolor{sywStampLightRed}{rgb}{0.90,0.74,0.74}

% Generate the stamp on the first page
\ifAddStamp
  % No-op offsets. Override these for, e.g.,
  % specific documentclasses that require a
  % different default stamp position.
  \newcommand{\syw@stampXOffset}{0.00}
  \newcommand{\syw@stampYOffset}{0.00}

  % Define the stamp
  \newcommand{\syw@stamp}{%
    \pgfmathsetmacro{\sr}{0.50}%
    \pgfmathsetmacro{\tr}{1.33*\sr}%
    \pgfmathsetmacro{\vr}{0.15}%
    \pgfmathsetmacro{\sd}{2*\sr}%
    \pgfmathsetmacro{\sx}{\syw@stampX + \syw@stampXOffset}%
    \pgfmathsetmacro{\sy}{\syw@stampY + \syw@stampYOffset}%
    \pgfmathsetmacro{\tx}{\tr*sin(\syw@stampAngle)}%
    \pgfmathsetmacro{\ty}{-\tr*cos(\syw@stampAngle)}%
    \pgfmathsetmacro{\vx}{\vr*sin(\syw@stampAngle)}%
    \pgfmathsetmacro{\vy}{-\vr*cos(\syw@stampAngle)}%
    \pgfmathsetmacro{\invsz}{1/\syw@stampSize}%
    \scalebox{\syw@stampSize}{%
      \href{\syw@url/tree/\syw@sha/}{%
        \begin{tikzpicture}[remember picture,overlay]
          \node (STAMP) at ($\invsz*(current page.north east) - \invsz*(\sx in, \sy in)$)
            [rotate=\syw@stampAngle]
            {\includegraphics[width=\sd in]{showyourwork-stamp.pdf}};
          \node (VERSION) at ($(STAMP.center) - (\vx in, \vy in)$)
            [rotate=\syw@stampAngle,font=\fontsize{5}{7}\selectfont\ttfamily\bfseries,color=sywStampLightRed]
            {\syw@stampVersion};
          \draw[draw=none,
            postaction={decorate},
            decoration={text along path,
              text={|\ttfamily\normalsize\bfseries|\syw@stampText},
              text align=center,
              text color=sywStampRed
            }]
            ($(STAMP.center) - (\tx in, \ty in)$)
            arc
            [start angle={\syw@stampAngle+90},
            end angle={\syw@stampAngle+450},
            radius=\tr in];
        \end{tikzpicture}%
      }%
    }%
  }
  % Render it as a background image on current page
  \AddToShipoutPictureBG*{
    \makeatletter%
    \syw@stamp%
    \makeatother%
  }
\fi

% Custom margin icon
\newcommand\marginicon[1]{
  \renewcommand\showkeyslabelformat[1]{#1}%
}

% User-facing commands
\newcommand\GitHubURL{\syw@url}
\newcommand\GitHubSHA{\syw@sha}
\newcommand\GitHubIcon{\faGithub\xspace}

% Figure script icon
\newcommand\syw@Script[1]{%
  \raisebox{0pt}[6pt][0pt]{%
    \href{\syw@url/blob/\syw@sha/\usevalue{#1}}{%
      \color{github-icon}\faGithub%
    }%
  }%
}

% Figure dataset icon
\newcommand\syw@DatasetOne[1]{%
  \raisebox{0pt}[6pt][6pt]{%
    \href{\usevalue{#1}}{%
      \color{dataset-icon}\faDatabase%
    }%
  }%
}

% Figure dataset icon
\newcommand\syw@DatasetTwo[1]{%
  \raisebox{0pt}[6pt][6pt]{%
    \href{\usevalue{#1}}{%
      \color{dataset-icon}\faDatabase%
    }%
  }%
}

% Figure dataset icon
\newcommand\syw@DatasetThree[1]{%
  \raisebox{0pt}[6pt][6pt]{%
    \href{\usevalue{#1}}{%
      \color{dataset-icon}\faDatabase%
    }%
  }%
}

% Figure cache icon
\newcommand\syw@Cache[1]{%
  \raisebox{0pt}[6pt][6pt]{%
    \IfSubStr*{\usevalue{#1}}{sandbox}{%
      \href{\usevalue{#1}}{%
        \color{sandbox-icon}\faRecycle%
      }%
    }{%
      \href{\usevalue{#1}}{%
        \color{cache-icon}\faRecycle%
      }%
    }%
  }%
}

% Variable script icon: links to a line in the Snakefile
\newcommand\syw@Variable[1]{%
  \raisebox{0pt}[6pt][0pt]{%
    \href{\syw@url/blob/\syw@sha/\usevalue{#1}}{%
      \color{github-icon}\faGithub%
    }%
  }%
}

% Set the graphics path for all figures
\graphicspath{{./}{./figures/}}

% Alias of \input for syw-controlled files
\newcommand\variable[1]{%
  \input{#1}\unskip\label{#1}\unskip%
}

